Improving SAM Requires Rethinking its Optimization Formulation

This paper rethinks Sharpness-Aware Minimization (SAM), which is originally formulated as a zero-sum game where the weights of a network and a bounded perturbation try to minimize/maximize, respectively, the same differentiable loss. To fundamentally improve this design, we argue that SAM should instead be reformulated using the 0-1 loss. As a continuous relaxation, we follow the simple conventional approach where the minimizing (maximizing) player uses an upper bound (lower bound) surrogate to the 0-1 loss. This leads to a novel formulation of SAM as a bilevel optimization problem, dubbed as BiSAM. BiSAM with newly designed lower-bound surrogate loss indeed constructs stronger perturbation. Through numerical evidence, we show that BiSAM consistently results in improved performance when compared to the original SAM and variants, while enjoying similar computational complexity. Our code is available at https://github.com/LIONS-EPFL/BiSAM.

==> Finetuning.tex <==
\section{Finetuning}
Finetuning on the valid dataset which is composed of a random subset of 10\% of the usual CIFAR10 training samples.

\begin{table}[H]
    \centering
    \caption{MetaOptSAM (400 epochs)}
    \begin{tabular}{C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}}
\toprule
\bm{$\rho$} & \bm{$1e-5$} & \bm{$1e-4$}  & \bm{$0.001$}  & \bm{$0.01$} &  \bm{$0.05$} & \bm{$0.1$}  & \bm{$0.2$} & \bm{$0.5$} & \bm{$0.8$}  & \bm{$1$} & \bm{$2$}    \\
\midrule                                                                 
       lr=0.1   &   97.02  &   97.06    &   97     &     96.82     &  97.08    &	97.2	&  97.1  & 97.22, 97.16, 97.12	& 97.24, 97.16, 97.24	& 97  & 96.86 	\\
       lr=0.05   &    &    96.64   & 96.94    &       & 		&     &		&   & 	&	&    
      \\
\bottomrule
    \end{tabular}
    \label{tab:metaoptsam-valid}
\end{table}


\begin{table}[H]
    \centering
    \caption{MetaSAM (200 epochs)}
    \begin{tabular}{C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}}
\toprule
\bm{$\rho$} & \bm{$1e-5$} & \bm{$1e-4$}  & \bm{$5e-4$} & \bm{$0.001$} & \bm{$0.005$}  & \bm{$0.01$} &  \bm{$0.1$}     \\
\midrule                                                                 
       lr=0.1   &  96.78   &  96.8, 96.76 &  96.74, 96.8  & 96.58, 97.08    &    &  95.7    &  /   	\\
       lr=0.05   &    &      & 96.62  &  96.7    &  96.14  &  95.3      &     		\\	
       lr=0.03   &    &      &   &   96.3   &   95.58    &     	\\
\bottomrule
    \end{tabular}
    \label{tab:metasam-valid}
\end{table}






\begin{table}[h]
    \centering
    \caption{OptSAM (400 epochs)}
    \begin{tabular}{C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}}
\toprule
\bm{$\rho$} & \bm{$0.01$} & \bm{$0.05$} & \bm{$0.1$}  & \bm{$0.5$}  & \bm{$1$}    \\
\midrule                             
       lr=0.1  & 97.02 &  96.76  &  97.16, 96.9, 97  &    97.04   &    96.74    		\\
       lr=0.05 & 96.94  &  97.02  &  96.82, 97.24, 97.04   &  96.98     &       	\\
       lr=0.03 &    &    &  97.04   &       &        	\\
\bottomrule
    \end{tabular}
    \label{tab:optsam-valid}
\end{table}


\begin{table}[h]
    \centering
    \caption{AOptSAM (400 epochs)}
    \begin{tabular}{C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}}
\toprule
\bm{$\rho$} & \bm{$0.01$} & \bm{$0.05$} & \bm{$0.1$}  & \bm{$0.5$}  & \bm{$1$}    \\
\midrule                             
       lr=0.1  & 96.98 & 97.06  & 96.92  &   97  &      /		\\
       lr=0.05 &  97.1 & 97.02  & 97.14  & 97.22  &    /   	\\
\bottomrule
    \end{tabular}
    \label{tab:aoptsam-valid}
\end{table}


\begin{table}[H]
    \centering
    \caption{SaddleSAM (400 epochs)}
    \begin{tabular}{C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}}
\toprule
\bm{$\rho$} & \bm{$0.01$} & \bm{$0.05$} & \bm{$0.1$}  & \bm{$0.5$}  & \bm{$1$}    \\
\midrule                             
       lr=0.1  & 96.7 &   96.88 &  97, 96.98  &   96.72    &     		\\
       lr=0.05 &  96.86 &  96.86  &  96.86  &  96.94    &       	\\
\bottomrule
    \end{tabular}
    \label{tab:saddlesam-valid}
\end{table}


\begin{table}[H]
    \centering
    \caption{PSaddleSAM (200 epochs)}
    \begin{tabular}{C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}}
\toprule
\bm{$\rho$} & \bm{$0.01$} & \bm{$0.05$} & \bm{$0.1$}  & \bm{$0.5$}  & \bm{$1$}    \\
\midrule                             
       lr=0.1  & 96.7 &  96.68  &  96.9  & 96.6     &     		\\
       lr=0.05 &   &  96.46  &  96.56  &      &       	\\
\bottomrule
    \end{tabular}
    \label{tab:psaddlesam-valid}
\end{table}


\begin{table}[H]
    \centering
    \caption{OptSAM2 (400 epochs)}
    \begin{tabular}{C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}}
\toprule
\bm{$\rho$} & \bm{$0.01$} & \bm{$0.05$} & \bm{$0.1$}  & \bm{$0.5$}  & \bm{$0.8$} & \bm{$1$}    \\
\midrule                             
       lr=0.1  &  &  97.08  &  97.16  &   97.04  & 96.9  &   97.22, 97.28    		\\
       lr=0.05 &   &  97.02  &  96.94   &  97.1  & 97.22, 97.06  &   97.1    	\\
\bottomrule
    \end{tabular}
    \label{tab:optsam2-valid}
\end{table}

\begin{table}[H]
    \centering
    \caption{OptSAM3 (400 epochs)}
    \begin{tabular}{C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}|C{1cm}}
\toprule
\bm{$\rho$} & \bm{$0.01$} & \bm{$0.05$} & \bm{$0.1$}  & \bm{$0.5$}  & \bm{$0.8$}  & \bm{$1$}    \\
\midrule                             
       lr=0.1 & 96.92  &    &  96.98, 97.06  &   97.12    &  97.24, 97.06  & 97.04 	\\
       lr=0.05 & 96.76  & 96.98   &  96.84, 97.04  &  97.24, 96.92  & 96.96   &  97.06    	\\
\bottomrule
    \end{tabular}
    \label{tab:optsam2-valid}
\end{table}

